Lagrangian Approaches for a class of Matching Problems in Computational Biology

This paper presents efficient algorithms for solving the problem of aligning a protein structure template to a query amino-acid sequence, known as protein threading problem. We consider the problem as a special case of graph matching problem. We give formal graph and integer programming models of the problem. After studying the properties of these models, we propose two kinds of Lagrangian relaxation for solving them. We present experimental results on real life instances showing the efficiency of our approaches.

==> NOUVEAUTE <==
septembre 1997 :
  -autres modifs : voir changes dans le fichier RR.dtx.

10 septembre 1997 : v3.4
- prise en main par Jose Grimm, a la place de Ph. Louarn
- suppression d'un tiret entre Sophia et Antipolis
- ajout de macros qui testent que l'argument de \RRtheme est correct.
- ajout de macros qui mettent un resume/abstract/motcle/keyword par defaut


08 septembre 1997 : v. 3.3
- no de telephone et fax national / international
- utilisation du package graphicx au lieu de epsfig

29 octobre 1996 : v. 3.2b
- no de téléphone à 10 chiffres

11 juillet 1996 :  v 3.2a
- à la demande de l'Ucis, la commande \RRno est rendue inactive.

06 juin 1996 : v3.2
- suppression de RRNo ==> no= ???? par defaut
- correction d'un bug dans RRA4 ==> centrage de l'adresse de l'UR dans la 
  page de titre

28 mars 1996 : v 3.1
correction de bugs : 
- cas de 2 themes differents
- appel de note dans les thanks

12 mars 1996 : v 3.0
Changement du n° d'ISSN des RT
Remplacement des programmes Inria par les thèmes.
Adaptation à LaTeX2e
Nouvelle adresse pour l'UR Rhône-Alpes
Maquettes Frame pour FrameMaker 5
Suppression des styles PI (locaux à l'Irisa).
Le style "french" ne fait plus partie de la distribution. Il doit
être récupéré à part...

29 juillet 1994 :
Nouveaux style PIA4 et RRA4 qui permette d'occuper plus de surface
sur la papier.

27 juillet 1994 :
Prise en compte de la notion de chapitre

06 avril 1994 :
Meilleure prise en compte de la charte graphique Inria





==> decompos.tex <==
\subsection{Problem decomposition}
The aim of cost-splitting techniques is to decompose a problem into subproblems of reasonable complexity. In our case, each subproblem should be a set of independent sheaves and single links. Several such decompositions exist, but the choice of a particular decomposition may impact a lot on performance: with a lot of subproblems, each one is simpler to solve, but it takes more subgradient iterations to reach a complete agreement between subproblems. Experimentally, the
following decomposition appears to be suitable and is easy
to obtain. 

First all $(i,i+1)$ links ($i \in [1,m]$) are put in $L^1$ subproblem (if one of them, doesn't exist, it is added with a corresponding null cost matrix). All vertex costs $c_i$, $i \in [1,m]$ are affected to $L^1$ subproblem. Thus, all other subproblems have null vertex cost.
 
Then, given $K$ a set of links we note $K^j$ the maximal subset of $K$ with
right end of links in $[1,j]$. We select the subset of $K$ which includes all the compatible
independent sheafs built from right to left. That is, if $K^j\neq\emptyset$,  let $s=max\{i|\exists (r,i)\in K^j\}$,
   then let $s'=max\{r|(r,s)\in K^j\}$ and $K^j_{rms} =\{(s',r)\in K^j\}  $. $K^j_{(s',s)}$ 
is the right most sheaf subset  (see Figure~(\ref{fig:rmsheaf})).
\begin{figure}[t]
  \begin{minipage}[c]{.40\textwidth}
~

  \epsfig{figure=rmsheaf.eps,scale=.40}
  \end{minipage}
\hfill
  \begin{minipage}[c]{.35\textwidth}
    \begin{eqnarray*}
K^{14}_{rms}&=&\{(11,13),(11,14)\}\\
K^{11}_{rms}&=&\{(5,8),(5,9)\} \\
K^{5}_{rms}&=&\{(2,5)\} \\
sss(K)&=&K^{5}_{rms}\cup K^{11}_{rms}\cup K^{14}_{rms}
    \end{eqnarray*}





  \end{minipage}

  \caption{The right most sheaf of $K^j$}
  \label{fig:rmsheaf}
\end{figure}
We can now define formally $sss(K)$ the subset of sheaves:
\begin{eqnarray*}
sss(K)= \emptyset& if& K=\emptyset \\ 
sss(K)= sss(K^{s'})\cup K^j_{(s',s)}  &with& j=max\{k|\exists (i,k)\in K\}\\ 
\end{eqnarray*}
The partition $\cal{P}$ is built applying iteratively $sss$.
While
${\cal{P}}=(L^1\cup\ldots L^i) \neq L$, define $L^{i+1}= sss(L\backslash(L^1\cup\ldots L^i))$ and add $L^{i+1}$ in $~\cal{P}$. 


==> divers.tex <==
\begin{tabular}{l|rrrrr}
Size&3650&     3.48e+20& 1.37e+29& 8.95e+33 &2.07e+37\\
$Q_1$&290.49  &392.35 & 569.16 & 891.61 &1719.01\\
$Q_3$&428.97&  525.18 & 789.48 &1089.14 &1878.55
\end{tabular}
The five distribution tables for the template 1ASYA0

\begin{tabular}{r|rr|}\hline
\textbf{Size}&\textbf{$Q_1$}&\textbf{$Q_3$}\\\hline
3650&    290.49  &428.97\\
 3.48e+20& 392.35 &  525.18 \\
1.37e+29&  569.16 &  789.48 \\
8.95e+33 &891.61 &1089.14 \\
2.07e+37& 1719.01&1878.55\\\hline

\end{tabular}

